Multi-Agent Car Parking using Reinforcement Learning

As the industry of autonomous driving grows, so does the potential interaction of groups of autonomous cars. Combined with the advancement of Artificial Intelligence and simulation, such groups can be simulated, and safety-critical models can be learned controlling the cars within. This study applies reinforcement learning to the problem of multi-agent car parking, where groups of cars aim to efficiently park themselves, while remaining safe and rational. Utilising robust tools and machine learning frameworks, we design and implement a flexible car parking environment in the form of a Markov decision process with independent learners, exploiting multi-agent communication. We implement a suite of tools to perform experiments at scale, obtaining models parking up to 7 cars with over a 98.1% success rate, significantly beating existing single-agent models. We also obtain several results relating to competitive and collaborative behaviours exhibited by the cars in our environment, with varying densities and levels of communication. Notably, we discover a form of collaboration that cannot arise without competition, and a 'leaky' form of collaboration whereby agents collaborate without sufficient state. Such work has numerous potential applications in the autonomous driving and fleet management industries, and provides several useful techniques and benchmarks for the application of reinforcement learning to multi-agent car parking.

==> common/titlepage.tex <==
\makeatletter
\begin{titlepage}

    % do not show the assignment name for the dissertation
    {
        \textbf{\Huge \@title}\footnote{\url{https://github.com/omarathon/rl-multi-agent-car-parking}} \\[1.5cm]
    }
    
    \Large \textbf{\@author}\footnote{\texttt{omar.tanner@warwick.ac.uk}}\\
    Department of Computer Science \\
    University of Warwick \\

    % include the current date for the dissertation
    \today{}
    
    

    % \begin{adjustwidth}{-\oddsidemargin-1in}{-\rightmargin}
    %     \centering
    %     \includegraphics[width=\paperwidth]{../common/line.png}
    % \end{adjustwidth}

    \vspace*{-3.5cm}

\end{titlepage}
\makeatother

